MASKER: Masked Keyword Regularization for Reliable Text Classification

Pre-trained language models have achieved state-of-the-art accuracies on various text classification tasks, e.g., sentiment analysis, natural language inference, and semantic textual similarity. However, the reliability of the fine-tuned text classifiers is an often underlooked performance criterion. For instance, one may desire a model that can detect out-of-distribution (OOD) samples (drawn far from training distribution) or be robust against domain shifts. We claim that one central obstacle to the reliability is the over-reliance of the model on a limited number of keywords, instead of looking at the whole context. In particular, we find that (a) OOD samples often contain in-distribution keywords, while (b) cross-domain samples may not always contain keywords; over-relying on the keywords can be problematic for both cases. In light of this observation, we propose a simple yet effective fine-tuning method, coined masked keyword regularization (MASKER), that facilitates context-based prediction. MASKER regularizes the model to reconstruct the keywords from the rest of the words and make low-confidence predictions without enough context. When applied to various pre-trained language models (e.g., BERT, RoBERTa, and ALBERT), we demonstrate that MASKER improves OOD detection and cross-domain generalization without degrading classification accuracy. Code is available at https://github.com/alinlab/MASKER.

==> backup/fig_analysis_keyword.tex <==
\begin{figure}[t]
% \vspace{-0.2in}
\centering
\includegraphics[width=0.4\textwidth]{figures/analysis.pdf}
\caption{
Top 10 keywords according to the attention scores,
chosen by BERT and our method trained on Fine Food and tested on SST-2.
We highlight the sentiment-related keywords.
} \label{fig:comparison}
\vspace{-0.1in}
\end{figure}

==> backup/fig_effect.tex <==
\begin{figure*}[t]
% \vspace{-0.1in}
%
\centering
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{figures/open_world.pdf}
\caption{OOD samples} \label{fig:open_world}
\end{subfigure}~
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{figures/cross_domain}
\caption{Domain shift} \label{fig:cross_domain}
\end{subfigure}~
\begin{subfigure}{0.32
\textwidth}
\includegraphics[width=\textwidth]{figures/substitution}
\caption{Keyword substitution} \label{fig:substitution}
\end{subfigure}
\vspace{-0.05in}
\caption{
Empirical settings that might show the degraded performance of the keyword biased model. BERT is (a) over-confidence on OOD samples, (b) has a significant generalization gap on domain shift, and (c) shows a notable accuracy drop on keyword substitution.
} \label{fig:keyword-effect}
%
\vspace{-0.1in}
\end{figure*}


==> backup/fig_keyword_long.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/keywords.pdf}
\caption{Keywords by selection schemes}
\label{fig:keywordcomparison}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/analysis.pdf}
\caption{Keywords by training methods}
\label{fig:comparison}
\end{subfigure}
\vspace{-0.05in}
\caption{
(a) Top 10 keywords chosen by the frequency-based and attention-based selection schemes from Amazon 50 class reviews dataset. (b) Top 10 keywords chosen by the attention-based selection, by BERT and BERT+MASKER models, from Fine Food dataset. We highlight the sentiment-related keywords, \ie, the keywords which are generalizable among the task rather than the specific domain.
}\label{fig:keyword}
\vspace{-0.1in}
\end{figure}

==> backup/impact.tex <==
\section*{Broader Impact}

This paper focuses on addressing inputs from outside of training distribution by handling inherent bias in training data. Since our research is closely related to safety, reliability, and fairness of natural language processing (NLP), we expect our research to bring the following consequences:

\textbf{Focusing on the reliability of NLP models.}
While numerous research focuses on improving the performance of NLP models \citep{devlin2018bert, lan2020albert, liu2019roberta}, the reliability of NLP models is still under-explored.
However, models for real-world NLP tasks, \eg, machine translation \citep{wu2016google}, sentiment analysis \citep{alharbi2019twitter}, and fake news detection \citep{vlachos2014fact}, have to reliably handle out-of-distribution (OOD) or domain-shifted inputs.
We believe that our work illustrates the importance of the reliability of the models and motivates further development.

\textbf{Facilitating unsupervised debiasing researches.}
Biases in the training data can raise crucial ethical problems such as unfair discrimination on the basis of gender or race \citep{sheng2019woman,zhao2017men}.
Numerous works attempted to reduce biases in training data \citep{clark2019don,he2019unlearn}, but most of them require specific prior knowledge on the bias.
However, having prior knowledge of all latent biases underlying the dataset is infeasible. Therefore, the prior-knowledge-based approach to handle biases has limited applicability to real-world tasks. We show the \textit{unsupervised} way to find and address biases in the dataset, and we hope our work facilitates the research in this direction.


% \textcolor{red}{
% Language models are widely used in real-world applications, \eg, machine translation \citep{wu2016google}, sentiment analysis \citep{alharbi2019twitter}, and fake news detection \citep{vlachos2014fact}. However, learning an unbiased (or fair) model is challenging due to the inheritance of various types of biases in the training corpus \citep{crawford2017trouble}. For instance, gender or race biases can raise crucial ethics problems \citep{sheng2019woman,zhao2017men}. Numerous work attempted to reduce such biases \citep{clark2019don,he2019unlearn}, but most of them require specific prior knowledge on the bias. 
% \sj{However, having prior knowledge of every bias is impossible, and detecting and fixing biases in the dataset requires high-cost. Therefore, handling bias by using prior knowledge has an inherent limitation for applying to the real-world.}
% In this paper, we propose a technique to reduce the keyword bias, one of the most common types of bias, in an \textit{unsupervised} manner. We believe that our work would be a step toward building \textit{reliable} intelligence systems that deeply understand the context of language.
% }


% brown2020language

% Language models are widely used in real-world applications.
% Building a fair (or unbiased) model is challenging due to various biases in the training corpus. Biases are prevalent among real-world corpus, and it is likely to force models to learn undesirable stereotypes or prejudices \citep{crawford2017trouble}. For example, biases about gender or race in the corpus are well-known, and many researchers are dealing with these biases \citep{brown2020language, huang2019reducing, sheng2019woman}. However, addressing relatively unknown biases are more challenging, and sometimes it is impossible to catch it at the human level. As a result, it can cause catastrophic results on unexpected inputs such as out-of-distribution or domain-shifted samples. Therefore, we have to deal with biases in \textit{unsupervised} manner. MASKER finds spurious cues that models are relying on, in an unsupervised manner and offer the right way for training. We are looking forward to MASKER for debiasing models from numerous biases in the dataset, and having much smarter and reliable language models, which are one step closer to the real-world application.

% in society and industry. 


% But in the real world application, models always have to deal with unexpected inputs, and even with malicious inputs (\eg, keyword substitution mentioned in \ref{sec:keyword-effect}). This is a challenging task since it is impossible to train models with every corpus in the world. Even collecting all the corpus in the world is possible, it is nonsense to assume there is absolutely no bias in the whole corpus. Therefore, debiasing models with given inputs are a very important task for the further improvement of the desirable language models.
% By applying MASKER, we are looking forward to having much smarter and reliable language models, which are one step closer to the real world application.




==> backup/motivation.tex <==
\vspace{-0.05in}
\section{Keyword bias}
\vspace{-0.05in}
\label{sec:motivation}

In this section, we explore the \textit{keyword bias} problem of the text classifiers.
In Section \ref{sec:keyword-bias}, we verify that the text classifiers are often biased to the shortcuts (\ie, keywords).
In Section \ref{sec:keyword-effect}, we discuss the empirical settings that keyword bias might degrade the reliability of text classification.

\vspace{-0.025in}
\subsection{Keyword bias in text classification}
\vspace{-0.025in}
\label{sec:keyword-bias}

We first empirically show that the text classifiers, even those built upon the pre-trained language models, are often biased to the shortcuts, which we call the \textit{keywords}. 
To verify this,
we fine-tune the BERT \citep{devlin2018bert}, arguably the most popular pre-trained language model, to Amazon 50 class reviews \citep{chen2014mining} dataset and select keywords from the attention (see Section \ref{sec:keyword-selection}).

Figure \ref{fig:bias} shows the frequency of the keywords under various settings. In Figure \ref{fig:bias_id} and Figure \ref{fig:bias_ood}, we select six keywords from the Amazon 50 class reviews dataset \citep{chen2014mining}. The frequency of each keyword is measured on (a) the same dataset, and (b) the 20 Newsgroups dataset. In (a), the keywords appear with high frequency from the keyword-relevant classes, \eg, the keyword for `computer' is found frequently in both `computer' and `monitor.' In (b), however, we find that the keywords \textit{also} appear frequently in OOD classes, \eg, the keyword for `iron' is frequently found in `autos.' In such cases, the OOD sample may be classified as an in-distribution with high confidence. Figure \ref{fig:bias_dg} shows the frequency of the keywords from sentiment analysis datasets, in other sentiment analysis datasets of different domains (\ie, cross-domain). In this case, we find that the keywords from one domain often do not generalize to other domains: non-diagonal terms are much lower than diagonal terms. Then, the model may fail to generalize to cross-domain samples not containing the exact keywords.


\vspace{-0.025in}
\subsection{Side effects of the keyword bias}
\vspace{-0.025in}
\label{sec:keyword-effect}

\input{resources/fig_effect}


The keyword biased model can introduce severe problems to the text classification. In particular, we consider three settings: out-of-distribution, domain shift, and keyword substitution.

First, we consider the out-of-distribution (OOD) scenario, where the OOD samples contain the overlapping keywords of in-distribution (ID) samples. We conduct experiments on 20 Newsgroups \citep{lang1995newsweeder} and Amazon 50 class reviews \citep{chen2014mining}, where we use a subset of classes as ID samples and the other classes as OOD samples. Figure \ref{fig:open_world} shows that BERT makes high-confidence predictions on OOD samples. See Section \ref{sec:exp_open_world} for the detailed experiment setting and more experimental results.

Second, we consider the domain shift scenario, where test samples share similar contexts with training samples but are less likely to contain the keywords from the training dataset. We conduct experiments on sentiment analysis datasets; train a model on Fine Food \citep{mcauley2013amateurs} and test the model on the IMDB \citep{maas2011learning} and SST-2 \citep{socher2013recursive}. Figure \ref{fig:cross_domain} shows that BERT has a significant generalization gap under domain shift. See Section \ref{sec:exp_cross_domain} for the detailed experiment setting and more experimental results.

Finally, we consider the keyword substitution scenario, that an adversary substitutes keywords to keywords for another class. Assume that an adversary changes the keyword `Apple' to `Google' while keeping the contexts. Then the reliable classifier should not predict it as a class `Google.' We conduct experiments on Amazon 50 class reviews, changing the keywords to the keywords of different classes. Figure \ref{fig:substitution} shows that BERT shows a notable accuracy drop on keyword substitution.


















==> backup/tab_cross_domain_mnli.tex <==
% \begin{table*}[t]
% \centering
% \caption{
% Cross-domain generalization results on MNLI tasks. We follow the settings of \citep{hendrycks2020pretrained}.
% }
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
% \multirow{3}{*}{Model} & \multicolumn{3}{c}{Telephone} \\
%  & \makecell{Telephone\\(ID)} & \makecell{Letters\\(OOD)} & \makecell{Face-to-Face\\(OOD)} \\ \hline
%     BERT & 80.5 & 77.4 & 77.5 \\
%     BERT+MASKER & 80.2 & 80.4 & 78.5 \\ \hline
%     RoBERTa & 84.8 & 83.6 & 83.5 \\
%     RoBERTa + MASKER & 86.0 & 85.9 & 83.8 \\ \hline
%     AlBERT & 82.9 & 82.8 & 80.9 \\
%     AlBERT+MASKER & & & \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

==> backup/tab_cross_domain_stsb.tex <==
\begin{table*}[t]
\centering
\caption{Cross-domain generalization results on STS-B tasks. We follow the settings of \citep{hendrycks2020pretrained}}
\label{tab:dg_sts}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|cc|c|c|c}
\toprule
\multirow{2}{*}{Train} & \multirow{2}{*}{Test} & \multirow{2}{*}{OpenMax} & \multirow{2}{*}{DOC} & \multicolumn{3}{c}{Vanilla/Residual/MASKER}\\
& & & & BERT & RoBERTa & AlBERT \\ \cmidrule{1-7}

\multirow{2}{*}{Images} & Images & xx.x & xx.x & xx.x/xx.x/xx.x & xx.x/xx.x/xx.x & xx.x/xx.x/xx.x\\
& MSRvid \\
\multirow{2}{*}{MSRvid} & MSRvid \\
& Images \\
\multirow{2}{*}{Headlines} & Headlines \\
& MSRpar \\
\multirow{2}{*}{MSRpar} & MSRpar \\
& Headlines \\

\bottomrule

\end{tabular}}
\end{table*}
